Exploring Modern GPU Memory System Design Challenges through Accurate Modeling

This paper explores the impact of simulator accuracy on architecture design decisions in the general-purpose graphics processing unit (GPGPU) space. We perform a detailed, quantitative analysis of the most popular publicly available GPU simulator, GPGPU-Sim, against our enhanced version of the simulator, updated to model the memory system of modern GPUs in more detail. Our enhanced GPU model is able to describe the NVIDIA Volta architecture in sufficient detail to reduce error in memory system even counters by as much as 66X. The reduced error in the memory system further reduces execution time error versus real hardware by 2.5X. To demonstrate the accuracy of our enhanced model against a real machine, we perform a counter-by-counter validation against an NVIDIA TITAN V Volta GPU, demonstrating the relative accuracy of the new simulator versus the publicly available model. We go on to demonstrate that the simpler model discounts the importance of advanced memory system designs such as out-of-order memory access scheduling, while overstating the impact of more heavily researched areas like L1 cache bypassing. Our results demonstrate that it is important for the academic community to enhance the level of detail in architecture simulators as system complexity continues to grow. As part of this detailed correlation and modeling effort, we developed a new Correlator toolset that includes a consolidation of applications from a variety of popular GPGPU benchmark suites, designed to run in reasonable simulation times. The Correlator also includes a database of hardware profiling results for all these applications on NVIDIA cards ranging from Fermi to Volta and a toolchain that enables users to gather correlation statistics and create detailed counter-by-counter hardware correlation plots with minimal effort.

==> exploration.tex <==

\section{Design Space Exploration}
\label{sec:design-space-expl}

In this section, we analyze the impact of our new memory system modeling.
In simulation, we study detailed memory system characteristics of
GPGPU workloads on a Pascal P102 architecture with GDDR5X DRAM.
%baseline that we have validated
%against real hardware in the previous section.

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/dram-read-transactions_html_1B-3_x-PASCALTITANX_1B-TITANX-P102-copyk.pdf}
    \caption{DRAM reads for New-Model versus silicon Pascal TITAN X\label{fig:dram-reads-correl}.}
\end{figure}


%We characterize our workloads into three different
%categories,
%cache-sensitive workloads (\textit{C-type}),
%streaming memory intensive workloads (\textit{M-type})
%and regular balanced workloads (\textit{B-balanced}).

%\begin{table}
% \begin{adjustwidth}{-.5in}{-.5in}
%  \begin{center}
%     \tiny
%    \scriptsize
%   \caption{Workloads used in this study} \label{table:workloads}
%    \begin{tabular}{|l|c|c|}
%        \hline
%        workload & type & input size \\\hline
%        BLK & M-type & 320 MB \\\hline
%        CONV & M-type & 16 MB \\\hline
%        FWT & M-type & 32 MB \\\hline
%        SP & M-type & 120 MB \\\hline
%        TRA & M-type & 16 MB \\\hline
%        VecAdd & M-type & 40 MB \\\hline
%        STREAM & M-type & 20 MB \\\hline
%        Copy  & M-type & 20 MB \\\hline
%        MiniFe  & M-type & 356 MB \\\hline
%        spmv  & C-type & 10 MB \\\hline
%        AMR  & C-type & 25 MB \\\hline
%        Join  & C-type & 8 MB \\\hline
%        bc  & C-type & 15 MB \\\hline
%        color\_max & C-type & 47 MB \\\hline
%        fw  & C-type & 200 MB \\\hline
%        mis  & C-type & 200 MB \\\hline
%        pagerank & C-type & 13 MB \\\hline
%        sssp  & C-type & 60 MB \\\hline
%        sssp\_ell  & C-type & 60 MB \\\hline
%        bfs  & C-type & 40 MB \\\hline
%        MM  & B-type & 32 MB \\\hline
%        HS  & B-type & 32 MB \\\hline
%        srad\_v1 & B-type & 6 MB \\\hline
%        srad\_v2  & B-type & 16 MB \\\hline
%        cns  & B-type & 64 MB \\\hline
%        Xsbench & B-type & 20  MB \\\hline
%        lulesh & B-type & 100 MB \\\hline
%    \end{tabular}
%  \end{center}
%\end{table}

\subsection{Cache Analysis \label{sec:cache-ana}}

\begin{figure*}
    \centering
    \includegraphics[width=180mm]{figs/l2cache_perf.pdf}
    \caption{Normalized performance improvement caused by sectoring the L2 cache and improving the
    write policy.\label{fig:sector_l2cache_perf}.}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=180mm]{figs/l2_cache_reqreduced.pdf}
    \caption{L2 cache policy impact on DRAM requests normalized to the baseline non-sectored cache and na\"ive write policy\label{fig:l2_cache_reqreduced}.}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=180mm]{figs/wasted_bw.pdf}
    \caption{Memory bandwidth utilization, broken down into the reasons for inactivity.\label{fig:wasted_bw}.}
\end{figure*}

In this subsection, we analyze the impact of the sectored L2 cache
with lazy fetch-on-read compared to the existing GPPGU-Sim 3.x
cache with a na\"ive write policy that fetches cache lines on write requests to fill them.
%This is what GPGPU-Sim 3.x does.
As shown in Figure~\ref{fig:sector_l2cache_perf},
sectoring the L2 and changing the write policy improves
the performance of our applications by 8\%.
The degree of performance improvement varies greatly and some
applications show a performance degradation.
Apps that show a slowdown with the improved L2 cache benefit from the
larger spatial locality of the non-sectored cache~\cite{rhu2013locality}.
The irregular workloads, such as BFS and spmv, and write intensive
workloads show a high performance improvement
with the sectored and lazy-fetch-on-read L2 cache.
Figure~\ref{fig:l2_cache_reqreduced} shows the reduction of
dram memory requests received from the L2 cache.
The figure shows a significant reduction in dram
requests, which translates to an energy and power
reduction as well.
On average, a 36\% reduction was observed
when applying the optimized L2 cache.



%Akshay: Can we show the HW value for reference?
%Its not clear what's meant by L2 cache performance



%\subsection{Memory Characteristics Analysis}

%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/latency_sens.pdf}
%    \caption{Latency Sensitivity\label{fig:latency_sens}.}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/bw_sens.pdf}
%    \caption{Bandwidth Sensitivity\label{fig:bw_sens}.}
%\end{figure}

%First, we study the latency and bandwidth sensitivity on a wide range of workloads.
%Figure~\ref{fig:latency_sens} depicts the latency sensitivity of all our apps.
%The majority of workloads are insensitive to memory latency, except for a few.
%Akshay: Previously we said all workloads have data set 2x of L2 cache
%The workloads reduction, b+tree and nw have small input size that fits in the L2 cache and show high hit rate at L2. Thus, they are sensitive to the cold misses that occur at the beginning of the kernel and thereby sensitive to latency. Figure~\ref{fig:bw_sens} depicts the bandwidth sensitivity on a wide range of GPGPU workloads. In this experiment, while we increase the memory bandwidth, we also increase the interconnection bandwidth to ensure we have enough throughput to sustain the memory requests from dram to cores. As shown in figure, the majority of workloads are sensitive to bandwidth. Increasing the memory bandwidth by 2X and 4X leads to 2.5X and 3.1X geometric mean performance improvement respectively.
%Akshay: Looks like there are quite a few apps which see improvement at 0.5xBW
%Surprisingly, some cache sensitive workloads show a performance improvement when we decease the memory bandwidth, such as bc and pagerank. We notice that reducing the memory bandwidth for these workloads leads to increasing L2 cache hit rate. Our explanation to this behavior is that reducing the bandwidth leads to increasing the latency of memory request and thereby allows the data set to reside longer in the cache before eviction and thus alleviates the thrashing that may occur in these irregular cache-sensitive workloads ~\cite{rogers2012cache}.

%Akshay: The graphs need to be labeled
%\begin{figure*}
%    \centering
%    \includegraphics[width=180mm]{figs/RBL.pdf}
%    \caption{Row Buffer Locality\label{fig:RBL}.}
%\end{figure*}

%\begin{figure*}
%    \centering
%    \includegraphics[width=180mm]{figs/BLP.pdf}
%    \caption{Bank Level Parallelism\label{fig:BLP}.}
%\end{figure*}

%Figures~\ref{fig:RBL} and ~\ref{fig:BLP} depict the row buffer locality (RBL) and bank level parallelism (BLP)
%for our workloads. In addition, figure~\ref{fig:BLP} shows the BLP\_ready which
%measures the average number of banks that have ready requests.
%Ready request means that the row buffer of this request is opened.
%For example, BLP\_ready=2, means, on average, we always have two banks
%where each has a hit-buffer request that can be serviced right-away by
%sending a column read to the row buffer.
%Akshay: Can we put the apps together in these categories?
%As shown in the figures, GPGPU workloads come with diverse memory characteristics,
%High-RBL with High-BLP, High-RBL with Low-BLP
%and Low-RBL and High-BLP.
%Moreover, the BLP\_ready for many applications equals two.

\subsection{Memory Analysis}



\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/writebuffer-crop.pdf}
    \caption{Write Buffer Performance\label{fig:writebuffer_perf}.}
\end{figure}
\end{comment}



Figure\ref{fig:wasted_bw} answers the question,
{\em where is memory bandwidth wasted?} In other words,
why are we are not able to achieve 100\% memory bandwidth utilization?
Based on our observations, there are four limiting factors that hinder
a bank to send a request to an opened row.
First, \textit{RCD}, which is defined as minimum number of clock
cycles required between opening a row of memory and accessing columns within it.
The \textit{RCD} is severe in applications that have high BLP and low RBL.
Second, read-to-write \textit{RTW} and write-to-read \textit{WTR} are other limiting factors.
Read-to-write and Write-to-read are the bus-turnaround penalty,
when switching from serving a read request to a write request, and vice
versa\cite{stuecheli2010virtual,stuecheli2010virtual,lee2010dram}.
The bus-turn-around delays are limiting factors in workloads that
are write-intensive, e.g. streaming workloads, wherein writes represent
more than 30\% of requests received by DRAM.
Third, command-command-delay \textit{CCDL} occurs when you read from
two banks that belong to the same bank group. In workloads that have
high bank-group-level parallelism, designing an intelligent memory
address mapping with advanced memory indexing\cite{zhang2000permutation}
can hide \textit{CCDL} delay.
%In our baseline architecture,
We choose the lower bits
of the bank\_Id as bank group index, since lower bits tend to have more entropy.
Further, we xor the bank\_Id bits with the lower
bits of row\_id to increase the bank-level
and bank-group-level parallelism\cite{zhang2000permutation}.

In figure\ref{fig:wasted_bw}, we characterize the wasted bandwidth
reasons on a wide range of workloads.
Although, we are using an advanced bank-group indexing,
many workloads are still limited by \textit{CCDL}.
On the workloads matvec, MM\_optimzed, SP and Xsbench,
nearly 20\% of bandwidth is wasted due to \textit{CCDL}.
\textit{RTW} and \textit{WTR} are also observed to be 
a bandwidth bottleneck for many streaming applications,
such as bfs, TRA, VecAdd, CONV, FWT, srad\_v2 and others.
In bfs, 40\% of bandwidth is wasted due to bus-turnaround time.



Many works have tried to address the bus-turnaround penalty
\cite{stuecheli2010virtual,stuecheli2010virtual,lee2010dram}.
Using separate read/write queues is a widely-used optimization technique
that splits read and write requests into different queues.
Write requests are buffered in a write queue and drained to DRAM
in a batch when the buffer reaches a specific threshold.
To study its effect on performance, we applied read/write buffer optimizations to our baseline.
We found that many workloads are insensitive to read/write buffer
optimization though they are bottlenecked by turn-around delay as
shown in figure\ref{fig:wasted_bw}.
Our investigation for these throughput workloads shows that,
there are many read requests pending in the banks' buffers when
the write buffer starts to drain the write requests.
These pending read requests interfere with write requests and
negate the read/write optimization. This behavior is unique to
throughput-oriented GPUs and does not occur as often in CPUs
that have few pending read requests at each banks' buffer when write drain starts.

%\subsection{HBM and GDDR5X Analysis}

%HBM\cite{hbmstandard2013high} and GDDR5X\cite{gddr5xstandard2013high} are two emerging DRAM memory
%technologies that support a high level of bandwidth compared to commodity DRR and GDDR5.
%The emerging memories come with new features and enhancements, such as per-bank
%refresh command and a dual-bus interface.
%In this subsection, we try to study  the new features and analyze their impacts on GPGPU workloads.

%\subsubsection{Per-bank refresh command}
%Since DRAM is based on dynamic cells, It requires periodic
%refresh operations to prevent data loss.
%It is well-known that DRAM refreshing causes a performance degradation and energy
%overhead\cite{agrawal2016clara,chang2014improving}.
%Typically, in commodity DRAM technology, refreshing is done at the rank-level
%(i.e., all banks within the rank are refreshed simultaneously and they are unavailable
%during the refresh time). It has been shown that the all-banks refresh policy has a
%huge performance and energy overhead on multi-core CPU. The per-bank (a.k.a. single-bank)
%refresh command is a new command that was firstly introduced in LPDDR3\cite{lpddr}
%to reduce memory refresh overhead.
%Instead of refreshing all banks, It refreshes a single bank
%at a time in a restrictive, sequential round-robin order.
%However, this restrictive order can refreshes a utilized bank
%that services a pending memory and prevents overlapping refreshes
%with accesses across banks\cite{chang2014improving}.
%GDDR5X and HBM support similar refresh mode with more flexibility
%and less restrictive ordering such that refresh commands can be issued to any banks in any order. Refresh overhead will be more critical in the future as HBM and GDDR5X continue to scale. There are high demands for larger memory size, especially from emerging workloads like Deep Learning\cite{rhu2016vdnn}. 

%We study the projection of refresh overhead on future HBM modules and see the effectiveness of single-bank refresh command. Table\ref{table:refresh} shows the expected refresh timing for future HBM. These numbers are adopted from\cite{hbmstandard2013high}. We implement three different refresh policies: (1) \textit{all-bank refresh} command that refreshes all banks at a time similar to commodity DRAM, (2) \textit{Round Robin} exploits the per-bank command in a restrictive round robin manner, (3) \textit{Greedy} harnesses the flexibility of HBM's per-bank refresh by refreshing banks that do not have pending request. Figure\ref{fig:refresh} shows the performance impact when applying the different refresh techniques compared to no-refresh on memory intensive workloads (M-type). As shown in figure, all-bank refresh has a severe impact on future modules, up to 6\%, 8\%, 11\%, 20\% performance loss was observed for 4Gb, 8Gb, 16Gb and 32 Gb respectively. Thanks to per-bank refreshing, the performance loss is mitigated and only 1\%, 1.2\%, 2\% and 3\% performance loss was observed with round robin scheduling. In fact, we do not observe a performance difference between applying round robin or greedy algorithm. This is because HBM modules has high number of memory banks (16-32 banks for 1Gb and 32 Gb respectively), thus the chance that the round-robin will refresh a utilized bank is very low. Moreover, as we observed in figure\ref{fig:BLP}, most of M-type workloads have BLP\_ready equals 2, which means on average, when memory is utilized, you always have at least two ready banks, so if you mistakenly refresh one of this bank in round-robin, the other ready bank will send its own request and thereby hide the refresh impact. It is important to note that while refresh does not seem to have a performance impact on future HBM, it may still cause a huge static energy consumption for periodically refreshing the rows and destroying row buffer locality. In this work, we do not implement energy model for Pascal architecture and HBM.
%We leave modeling the Energy model and studying the refreshing energy consumption for future work. 


%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/refresh.pdf}
%    \caption{Memory Refresh Impact\label{fig:refresh}.}
%\end{figure}

%\begin{table}
% \begin{adjustwidth}{-.5in}{-.5in}
%  \begin{center}
%     \tiny
%    \scriptsize
%   \caption{DRAM Refresh Timing} \label{table:refresh}

%    \begin{tabular}{|l|c|c|c|c|}
%        \hline
%        size & 4 Gb & 8 Gb & 16 Gb & 32 Gb \\\hline
%        refresh  & 1 row & 1 row & 2 rows & 4 rows\\\hline
%        tREFI & 128 cycles & 128 cycles & 128 cycles & 128 cycles \\\hline
%        tRFC & 48 & 72 & 96 & 120 \\\hline
%    \end{tabular}
%  \end{center}
%\end{table}

%\subsubsection{HBM Dual-bus interface}

%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/HBM-dual-interface.pdf}
 %   \caption{HBM Dual Interface\label{fig:HBM-dual-interface}.}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/dual_bus_eff.pdf}
%    \caption{dual bus efficiency\label{fig:dual_bus_eff}.}
%\end{figure}


%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/dual_bus_perf.pdf}
%    \caption{dual bus Performance Impact\label{fig:dual_bus_perf}.}
%\end{figure}

%Dual-bus interface is another feature that comes with HBM. In the new interface, column and row commands have separate buses such that column and row commands can be sent simultaneously to DRAM. %Figure\ref{fig:HBM-dual-interface} depicts the structure of dual-bus interface compared to single-bus interface that is used in commodity DRAM and GDDR5X. As shown in figure, 
%In single-bus interface, typically, column-to-column delay is two cycles (i.e. the data burst are sent over two cycles). Thus, there should be one cycle delay between every read/write column requests, and thereby row commands can be sent during this CCD delay cycle. In HBM, CCD equals one cycle. This is because the data bus width has increased to 128 bits and thereby reading 32 bytes requires only one cycle. Therefore, dual bus interface is used to send row command simultaneously with column command. This new interface can improve bandwidth utilization. Figure\ref{fig:dual_bus_eff} depicts the dual-bus efficiency which is measured as the percentage of the number when row and column are issued simultaneously on the dual-bus interface. %Figure\ref{fig:dual_bus_perf} shows normalized performance improvement when applying dual-bus interface. 
%It is observed that workloads that have High-BLP tend to have higher dual-bus efficiency and more performance improvement compared to other workloads.
%SP performance is increased by 6\% with dual-bus interface.

%\subsubsection{figs/GDDR5X Pseudo-independent Memory Accesses}

%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/GDDR5X_indpen_mem_access_reduced.pdf}
%    \caption{GDDR5X independent Memory access mode\label{fig:GDDR5X_indpen_mem_access}.}
%\end{figure}

%\begin{figure}
%    \centering
%%    \includegraphics[width=85mm]{figs/dram_reqs_on_real_HW.pdf}
%    \caption{DRAM reqs on real HW to demystify GDDR5X over-fetching \label{fig:dram_reqs_on_real_HW}.}
%\end{figure}

%GDDR5X\cite{gddr5xstandard2013high} minimum access granularity (a.k.a. atom size) is 64 bytes, whereas L2 cache sector size is 32 bytes. Im this case, L2 cache will read 64 bytes for every read request and thereby reduce sector cache efficiency. However, GDDR5X comes with new access mode, Pseudo-independent Memory Accesses, in which the memory controller can still issue two different 32-bytes accesses that belong to the same row page, such that one access is sent to any column at the lower part of the row page while the other is sent to any column column within that higher part of the page.
%Figure\ref{fig:GDDR5X_indpen_mem_access} depicts the pseudo-independent memory accesses mode.
%A smart memory controller is required to find and schedule two transactions in the buffer that satisfy the previous condition and reduce GDDR5X memory over-fetching. In order to study the impact of over-fetching on modern GPUs, we have run an irregular microbenchmark on different GPU hardware that employ GDDR5 as well as on Pascal TITANX P102 that uses GDDR5X.
%Figure\ref{fig:dram_reqs_on_real_HW} shows that, on GDDR5X there are more accesses than previous GDDR5-based GPUs. Our explanation is due to GDDR5X over-fetching. In fact, we find out that GDDR5x over-fetching is typically occurred in irregular workloads whereas regular workloads tend to have the expected number of accesses. Also, we observe that most of these over-fetching accesses are write accesses. In our baseline, we do not implement GDDR5X Pseudo-independent Memory access, instead we double the number of memory channels and decrease access atom\_size to 32 bytes. We leave modeling GDDR5X over-fetching and building a smart memory controller that exploits the new feature for future work. 




==> ispass2019-subm (2)/background.tex <==

%\section{Pascal Architecture}


==> ispass2019-subm (2)/conclusion.tex <==

\section{Conclusion }
\label{sec:conclusion}
This paper presents the most accurate open-source
model of a contemporary GPU to date.
Our detailed hardware characterization
and modeling effort decreases the execution time error
in GPGPU-Sim, the most popular GPU simulator in use today,
by $2.5\times$ when running
a comprehensive suite of contemporary workloads.
%The extensively validated memory system
%reduces error on key memory system counters by $66\times$.
Through our detailed micro-benchmarking and remodeling, we have uncovered a number of
important design decisions made in the GPU memory system that no
previous work has identified and no open-source simulator has attempted to model.
%The resulting simulator represents the
%most accurate GPU simulation to date, reducing error on a number of key
%memory system metrics by up to $24\times$.

The paper goes on to concretely demonstrates the effect this memory system error
has on design decisions.
Specifically, we show that error in the less detailed memory system model
discounts the performance effects of out-of-order memory
access scheduling, hampering potential research on the topic.
Conversely, the less detailed model over-estimates the
impact of L1 cache contention, as the throughput of the L1 cache is no longer
a bottleneck to the memory system in contemporary GPUs.

In the process of creating our detailed model, we created the {\em Correlator}
simulation and correlation infrastructure that can be easily used to
validate new modeling efforts as new hardware and simulation models are created.
We hope that releasing all the infrastructure used to perform this validation,
along with the more detailed model itself, will help facilitate the continued development of
simulation models that keep up with changes in contemporary
industrial designs so that academics can more accurately study what should
comes next.

%Both of these techniques would have been considered abstraction error in
%the less detailed model, as researchers would have given up on memory access scheduling
%and refined ideas around the L1 cache throughput bottleneck.

%To validate our model, we present the first counter-by-counter validation of an open-sourced GPU simulator. 
%This paper details the sources of error in the
%most widely used open-source GPU simulator, through a bottom-up micro-benchmarking process.
%In particular, we have demonstrated the pitfalls introduced by the generally-accepted
%methodology of scaling the existing simulation model to represent contemporary GPUs.
%To rectify this situation, we then redesign the memory system of
%the popular simulator, GPGPU-Sim to more accurately represent
%a contemporary Volta TITAN V GPU.



%Using the new model, we present a taxonomy of wasted bandwidth in the GPU memory system that can spur further research by identifying areas for improvement. Also, the Multichip module support enables us to reproduce work from an industrial simulator, thus advancing the state-of-the-art for open-source GPU simulations and gaining additional insights into the design of future GPUs.

==> ispass2019-subm (2)/correlation.tex <==
\section{Hardware Correlation}
\label{sec:hw-correl}

Throughout this section we will study the correlation of both the older, less detailed
GPGPU-Sim model and our enhanced version versus a silicon NVIDIA Volta TITAN V card.
The correlation figures presented throughout this section plot the collected hardware
number on the  x-axis and the GPGPU-Sim number on the y-axis.
Depending on the statistic, there are up to  \textasciitilde2400 datapoints (\~1200 kernels
with one data point for each of the old and new models) on each graph. 
The center of the larger orange circle represent the new GPU model and the small black
dot is the old model.
The {\em New Model} represents the results after performing the memory system
enhancements detailed in Section~\ref{sec:exp}, while the {\em Old Model} is our best-effort
attempt to model the Volta card using the existing codebase with only configuration file changes
to the existing GPGPU-Sim memory model. We note that both configurations make use of
the virtual PTX ISA, which is different from the SASS machine code used in the Volta.
Using PTX enables us to run many more workloads than with the limited support in GPGPU-Sim
for PTXPLUS. Moreover, recent work~\cite{jain2018quantitative} has demonstrated that while using PTXPLUS
can slightly improve the correlation of compute-intensive workloads, but has largely no effect on
memory-intensive applications and that error in the memory system is the most pervasive cause of error
in the simulator, independent of ISA choice.

This section begins by presenting the improvement in overall performance correlation
that results from our enhanced memory model. Then we detail how well the performance
counters in the memory system correlate to both the new and old models.
%with each dot representing one kernel launch from Rodinia 3.1~\cite{industry30}.
%We chose the Rodinia benchmark suite since it was used to validate GPGPU-Sim 3.x againstFermi. 
%To begin our correlation analysis, let us consider the sources of error in the existing GPGPU-Sim model:

%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/3-x-ptx-versus-ptxplus-crop.pdf}
%    \caption{Global memory transactions for GPGPU-Sim 3.x's PTX and PTXPlus, correlated to
%    the Pascal Titan X hardware on Rodinia kernels as demonstrated in %~\cite{jain2018quantitative}\label{fig:load-acc-ptxplus-correl}. }
%\end{figure}



\begin{comment}
\begin{itemize}
\item{ { \bf System-level effects }: The effects of 
kernel launch overhead, memory copies on L2 state,
the virtual memory system latency and thread-block work assignment are all
not modeled in GPGPU-Sim, which can have a significant impact on latency and execution cycles correlation.
}
\item{ { \bf Core bandwidth modeling} }: GPU cores have been modified
significantly since the Fermi architecture. The memory system in the core in
particular has changed in drastic ways. Some documented changes include the use
of a sectored, streaming and a
banked L1 cache with much higher throughput than that modeled in GPPGU-Sim.
\item{ { \bf Execution of a virtual ISA}: GPGPU-Sim, and most other open-source
simulators run a virtual ISA (PTX), since it is documented enough to create a functional 
model for.
Prior work~\cite{jain2018quantitative} has shown that modeling a machine ISA, which is 
implemented as PTXPlus in GPGPU-Sim, can improve the correlation of compute-intensive
workloads. However,~\cite{jain2018quantitative} also demonstrated that memory-intensive and
cache-sensitive applications were largely insensitive to ISA choice because of
excessive error in the memory system.
%Figure~\ref{fig:load-acc-ptxplus-correl} illustrates
%this point. The number of global memory transactions generated in the public version
%of the simulator is incorrect in both PTX and PTXPlus and is incorrect by roughly the same
%amount. Note that the improved modeling in our paper improves the correlation of
%global memory transactions in both PTX and PTXPlus.
%However, the use of PTX makes the modeling of instruction latency and throughput characteristics
%in the core difficult. On the other hand, running machine ISA (a.k.a. PTXPLUS) may provide accurate modeling and more correlation to the hardware~\cite{jain2018quantitative}. 
%However, Figure~\ref{fig:load-acc-ptxplus-correl} demonstrates
%that, although both PTX and PTXPlus have a high error rate in the public simulator due to
%inaccuracies in GPGPU-Sim's Pascal coalescing model, they are equivalent.
}
\item{ { \bf Inaccuracies in modeling throughput-oriented memory systems}:
Finally, several previous works have identified inaccuracies in the GPGPU-Sim memory
system~\cite{daidemand,nowatzki2014gem5,debunkinggpgpusim,nugteren2014detailed,jain2018quantitative}.
Given that the memory access stream of PTX instructions is reasonably accurate,
and that the memory system is a source of high error in the current GPGPU-Sim
model we focus our enhanced modeling efforts there.
}
\end{itemize}
\end{comment}

\subsection{Overall Cycle Correlation}

Figure~\ref{fig:cycles-correl} plots the resulting error and correlation of
cycles in both the old and new models. The error bars on the x-axis represent the
range of the silicon GPU execution time for this particular kernel over
10 successive runs of the application. To minimize the effect of
noisy, small kernels on the correlation results, only kernels that ran for at least 8000
GPU cycles in hardware are considered for cycles correlation.
Both the correlation mean absolute error of cycles are significantly
better using the new memory model. In particular, the mean absolute error is reduced by 
~$2.5\times$. This result confirms our working assumption that increasing the level of
detail in the memory system would decrease the overall error in execution time.
%Although overall correlation and accuracy are vastly improved and fairly good,
%there are still a few areas where the simulator can be 


\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/titanv-cycles-crop.pdf}
    \caption{Execution time correlation for the NVIDIA TITANV\label{fig:cycles-correl}. }
\end{figure}


\subsection{Correlating the L1}

By default the L1 cache is enabled in Volta (unlike in prior generations like Pascal, where the L1 cache was
shared with the texture and disabled by default).
Therefore; to run all of our test, we assume that the L1 is enabled and our newly implemented
adaptive L1/shared memory partitioning algorithm determines it's size. Independent of the number of
data lines allocated, we assume the streaming cache is still in use and that the number of tags are
available the same, even if more of the on-chip SRAM storage is devoted to shared memory.

Figure~\ref{fig:l1access-correl} plots correlation for the L1 read accesses
generated. Note that for all the counter correlation graphs, there are no errors on the hardware
measurement, as the hardware nvprof profiler runs the app several times to collect the statistics and
we have found these to be much more stable than execution time over successive runs of the apps.
Moreover, we plot the results for all the kernels run, regardless of their execution time,
as the counters are less noisy and more consistent than execution time.
As figure~\ref{fig:l1access-correl} shows, the error in the new model has been reduced to almost zero,
where the old model gives almost 50\%. This is primarily due to the implementation of
Volta coalescer and the fact that the L1 cache is sectored. The consistent band of accesses in the old model
at $y = 4x$ are reflective of this. 1 128B access in the old model will count as 4 sector
accesses in the new model. Completely divergent applications show consistent behaviour between both
models since 32 unique sectors are generated in the new model and 32 unique cache lines are generated
in the old model.


\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/l1readaccess-crop.pdf}
    \caption{ L1 read accesses correlation for the NVIDIA TITANV\label{fig:l1access-correl}. }
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/l1hitrate-crop.pdf}
    \caption{ L1 hit rate correlation for the NVIDIA TITANV\label{fig:l1hitrate-correl}. }
\end{figure}

Figure~\ref{fig:l1hitrate-correl} plots the corresponding hit rate for the L1 cache.
We note that this statistic is particularly hard to correlate, given that the warp scheduling
policy, cache replacement policy and hit/miss accounting decisions in the profiler can skew the results.
For example, the through rigorous microbenchmarking we determined that the hardware profiler
will count a sector miss on a cache line whose tag is already present as a "hit", but will still
send the sector access down to the L2. Effectively, the profiler appears to be counting 128B
line cache tag hits, even if the sector is still fetched and the instruction must wait.
Even with these variables, our improved cache model and coalescer achieve only 20\% error
(a 2$\times$ improvement over the old model) and a correlation of 93\%.
In the apps where pervasive error still exist, we believe more detailed
reverse engineering of the warp scheduling policy and L1 eviction policy would help.





\subsection{Correlating the L2}
\label{sec:l2-corr}

%In the Pascal Titan X, the default configuration disables the L1 cache, sending all accesses to the
%L2 in transactions of 32 bytes. This configuration provides a clean method to validate the L2 cache's
%behavior since we will not have any filtering or bandwidth limiting occurring at the L1. We start by correlating L2 read accesses.

To determine how well the memory system is operating at the memory controller
level, we begin by examining the performance of the memory-side L2 data cache.
Figure~\ref{fig:l2-read-correl} plots the correlation of L2 read accesses versus hardware.
Both correlation and error are much improved with the new model, with absolute error
reaching only 1.15\%. Interestingly, the relatively high
error in L1 miss rate does not end up resulting in error at the L2 level.
This leaves us to believe that most of the error is a result of accounting peculiarities
for L1 cache hits, like the sector miss situation described previously.

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/l2-read-transactions-crop.pdf}
    \caption{L2 read transaction correlation with NVIDIA TITAN V\label{fig:l2-read-correl}. }
\end{figure}

In terms of improvement over the old model, there is a significant fraction of
error coming from accessing 128B lines instead of 32B sectors from the L1,
again note the old model line at $y=4x$.
We also collected information on write transactions, and noticed similar behaviour
which is summarized in Table~\ref{ta:corr}.

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/l2-read-hits-crop.pdf}
    \caption{L2 read hit transaction correlation with NVIDIA TITAN V\label{fig:l2-read-hit-correl}. }
\end{figure}

We also attempted to correlate the L2 cache read hit rate with simulation results,
but found that the profiler gives inconsistent results, some of which are greater than 100\%.
So instead, we correlated with the number of L2 hits, which gave more grounded readings.
Figure~\ref{fig:l2-read-correl} presents the L2 read hit correlation.
Overall, the hit error is roughly the same as the error on the L1 cache, \~15\%.
Again, at the L2 scheduling effects from the order in which memory accesses reach the L2 will have an
effect on it's hit rate. The older model suffers significant error at the L2, even more than at
the L1 (80\% versus 40\%). Our model shows significantly better correlation for two primary several reasons.
First, since the number of accesses is more correlated the overall behaviour should be more similar.
Second, our model fills the L2 on memory copies from the CPU avoiding many unnecessary misses in the L2
when kernels with smaller data sets begin. The majority of excessively low old model points are
examples of this. We also collected data on the number of read hits, which showed a similar trend.

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/dram-read-transactions_html_TITANV-1B-FLUSHL1-COPYK_TITANV_OLD-1B-FLUSHL1-crop.pdf}
    \caption{DRAM read transactions correlation versus NVIDIA TITAN V\label{fig:dram-reads}.}
\end{figure}

%The mean absolute error across all kernels
%is 0.23\%. In contrast, the error on the current GPGPU-Sim model, when configured to match the Pascal
%Titan X is 47.72\%. 
%Akshay: Can we put this in methodology? Corr above 98% is not true with the updated data
%Note that throughout this paper we will not quote the correlation coefficient
%for any of the metrics we plot. The correlation coefficient for most of the statistics we plot
%in this paper is very high (in excess of 98\%). However, it can be a misleading metric, especially
%when attempting to correlate counters in throughput architectures. To illustrate this
%point, consider a simulator that consistently underestimates L2 traffic by $10\times$. The absolute 
%error for such a simulator would be 90\%, while the correlation coefficient will be 1.00.
%You may imagine the incorrect memory system design decisions that will be made with 10$\times$ less memory
%traffic.



%Figure~\ref{fig:l2-write-correl} plots the correlation of L2 write accesses.
%Here, we achieve 4.16\% error (compared to 50.91\% for 3.x). Even with our enhancements,
%the simulator is under estimating L2 writes in bands of 2 and 4 $\times$.
%A detailed micro-benchmarking of this phenomena, outlined in Section~\ref{sec:pascal-mem},
%reveals that the coalescer behaves differently than the documentation when dealing with divergent writes.
%Despite this minor error, the L2 write error remains very low and far better than GPGPU-Sim 3.x.


%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/l2-write-hits-crop.pdf}
%    \caption{L2 write hit correlation for NVIDIA TITANV\label{fig:l2-write-correl}. }
%\end{figure}

%Since reads are on the critical path and GPU benchmarks tend to be read-heavy, we focus the
%remainder of our correlation study on reads.
%Figure~\ref{fig:l2-hits-correl} plots the correlation of L2 read hits.
%Hits are a harder metric to match than accesses, since a number of second-order effects determine their
%accuracy, such as compiler instruction scheduling and hardware warp scheduling. We can see from the figure that our new model does a good job (13.76\% versus 55.33\% for 3.x)
%for larger benchmarks.
%However, when smaller kernels are run, the accuracy greatly
%diminishes. Detailed profiling reveals there are undocumented, system-level effects
%changing the content of the L2 cache. Applications that are composed of many, short running kernels
%are the cause of our inaccuracy below 1000 read hits. Further micro-benchmarking is required to
%determine the exact cause of L2 hit error for successive, cooperative kernel launches. %Also, supporting the new pascal machine instruction set (\textit{sm\_61}) can reduce the hit rate error further. \footnote{the current version of GPGPU-sim supports the old \textit{sm\_13} machine ISA}.

\subsection{Correlating DRAM}



Finally, Figure~\ref{fig:dram-reads} plots the correlation of DRAM read accesses.
The error rate here is 15\% (v.s. 89\% for the old model). As expected, small errors in the upper levels
of memory propagate into larger errors at the lower levels. The new model DRAM read correlation
remains high and is again more accurate for larger kernels. Interestingly, the reason for the massive error
in the old model was dues to its per-cacheline fetch on write policy
(detailed in Section~\ref{sec:memory-l2}). The end result of that policy was that every write to the
writeback L2 fetched 4 32-byte memory values from DRAM, which is why the DRAM reads of
the old model consistently are consistently overestimated. Our updated model has eliminated this problem
by sectoring the cache and implementing a more intelligent write policy, explained in Section~\ref{sec:memory-l2}.
We note that we only collect data here for kernels that have at least 1000 dram accesses, as we found the
counter values from hardware tended to be inconsistent at such small numbers and both the new and old
model resulted in massive amounts of error due to being off by relatively few memory accesses.

%\subsection{Correlation Summery}



%Since our work has focused on the memory system, in particular memory system accesses,
%we know that it will have some impact on overall performance and power correlations.
%As shown in Table~\ref{ta:corr}, our performance error does improve (from 55.55\%
%down to 46.32\%).
%However, it is still fairly high. There are several reasons for this, due to the other
%sources of error listed above. A more thorough analysis of in-core latencies, machine instruction set
%and kernel launch latencies should be performed to bring the timing more in-line with hardware.
%As for power, we anticipate that all the improvements in the energy-hungry memory system
%will reduce GPU-Wattch's \cite{leng2013gpuwattch} reliance on scaling co-efficients to estimate power as more of the
%GPU's architecture has been modeled.

==> ispass2019-subm (2)/demystifying.tex <==
\section{Exploring the Volta Memory System}
\label{sec:cache-demy}
The memory system in modern GPUs has changed significantly
since the last detailed modeling effort in GPGPU-Sim, which
took place for the Fermi architecture.
%The L2 cache size has increased from 768KB to 3 MB in Pascal 
%P102~\cite{pscalp102} and 4 MB in P100~\cite{pscalp100}.
%The role of L2 cache in a GPU is different from the CPU's last level cache.
Unlike in CPUs, the caches in GPUs are not primarily used to reduce 
single-thread memory latency, but rather
are designed as a bandwidth filter, reducing accesses to lower
levels of memory.
%as opposed to serving as a latency reduction mechanism
%increase the throughput of memory bandwidth,
%where the latency can be hidden by zero-overhead warps context %switching.
%Akshay: faster rate or throughput?
Workloads with a higher hit rate in the L2 cache service more requests at the faster throughput of the L2 cache,
which is typically 2X the {{DRAM}} throughput. There have been numerous works tried to demystify GPU architecture and memory system details through micro-benchmarks for Tesla GT200~\cite{wong2010demystifying}, Fermi~\cite{nugteren2014detailed}, Maxwell~\cite{mei2017dissecting}, and recently Volta~\cite{voltacitadel}. They demystified the L1/L2 cache's  associativity, replacement policy, indexing and capacity. However, none of these works dissect the details of Volta L1 streaming cache behaviour, adaptive cache configuration, sectoring L1/L2 caches, Volta coalescer and L2 write policy, taking into account that these details have a substantial impact on the GPU Modeling. In the following subsections, we explore the design of the Volta L1/L2 cache policy in order to accurately model the Volta memory system.

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/demystiying_coal.pdf}
    \caption{Volta coalescer micro-benchmark \label{fig:demystiying_coal}.}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/coal_strides_volta-crop.pdf}
    \caption{Volta coalescer micro-benchmark results\label{fig:coal_strides}.}
\end{figure}

\subsection{Volta Memory Coalescer \label{sec:pascal-mem}}
 
To understand the behaviour of the Volta global access coalescer,
we create the micro-benchmark shown in Figure~\ref{fig:demystiying_coal}.
We run our micro-benchmark on the NVIDIA
TITANV~\cite{titanv} and collect the
results via nvprof 10.0~\cite{nvprof}.
In the micro-benchmark, we adjust the number
of cache lines accessed by a warp based on variable {\em stride}.
When stride=1, each thread will access a different cache line,
when stride=8, each consecutive group of eight threads will access the same cache line, and so on.

Figure~\ref{fig:coal_strides} plots the number of L1 cache reads
and writes per warp.
In figure~\ref{fig:demystiying_l2write},
when stride=1, each thread reads a different cache
line, resulting in 32 accesses for each warp.
When the stride=32, the memory access is converged,
and all the threads within the same warp
will access the same cache line,
however we receive four read accesses at L1 cache,
as shown in figure.
This means that the access granularity of the L1 cache is 32B.
To determine if the cache has a true 32B line size or if
the line size is still 128B (the cache line size in
GPGPU-Sim's modeled Fermi coalescer is 128B), with 32B 
sectors~\cite{liptay2000structural,seznec1994decoupled}, we created
an additional microbenchmark. Our line-size-determining microbenchmark
fills the L1 cache, evicts one entry then attempts to re-access
the data loaded into cache. We find that the eviction granularity
of the cache is 128B, indicating that the L1 cache has 128B lines with
32B sectors.
Furthermore, the coalescer operates across eight threads, i.e. the 
coalescer tries to coalesce each group of eight threads separately to
generate sectored accesses.
%For writes, we notice different behavior. For all the strides,
%the writes have similar behavior to the reads,
%except when stride=8 and 12, the number of writes is greater than the number of reads
%(2X extra writes when stride=8).
%This means that the coalescer granularity is reduced to four threads,
%when the number of converged threads is less than 16.
%One explanation to this is because the global L1 cache and Tex cache are
%merged together in one structure in the Pascal P102.
%It is well known that texture cache coalesces at the granularity of four threads.
%It seems that the L1 cache and the texture cache P102 have different a different coalescer for reads,
%while they both share the same coalescer for writes.
We ran these same microbenchmarks with L1 bypassing
turned on and we observed similar behavior at the L2 for both reads
and writes, indicating that the L2 cache has a similar configuration.

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/demystiying_l2write.pdf}
    \caption{Microbenchmark to explore the Volta L2 cache write policy \label{fig:demystiying_l2write}.}
\end{figure}

\subsection{L2 cache \label{sec:memory-l2}}

Since high throughput memory systems are especially sensitive
to write traffic, the handling of writes at the L2 is very important.
The existing GPGPU-Sim memory model fetches 128B cache lines
from DRAM on write misses at the L2 and uses an allocate-on-fill
writeback policy.
To determine what the behaviour of writes at the L2 is in
real hardware, we created the small microbenchmark in Figure~\ref{fig:demystiying_l2write}.
%It is important to demystify the L2 cache policy to accurately model the L2 cache.
%From our observation on running a small micro-benchmark, we find out that L2 applies
%a write-back with write allocate policy.
The microbenchmark confirmed that the L2 is writeback with a 
write-allocate policy.
However, we observed some interesting, previously unmodeled behaviour
that occurs on write misses.
In literature, there are two different write allocation policies~\cite{jouppi1993cache},
\textit{fetch-on-write} and \textit{write-validate}.
In fetch-on-write, when we write to a single byte of a sector,
the L2 fetches the whole sector then merges the written portion to
the sector and sets the sector as modified.
In the write-validate policy, no read fetch is required,
instead each sector has a bit-wise write-mask.
When a write to a single byte is received,
it writes the byte to the sector, sets the corresponding write bit and 
sets the sector as valid and modified.
When a modified cache line is evicted, the cache line is written back to
the memory along with the write mask. It is important to note that,
in a write-validate policy,
it assumes the read and write granularity can be in terms of bytes
in order to exploit the benefits of the write-mask.
In fact, based on our micro-benchmark shown in 
Figure~\ref{fig:demystiying_l2write},
we have observed that the L2 cache applies something similar to
write-validate.
However, all the reads received by L2 caches from the coalescer are
32-byte sectored accesses. Thus, the read access granularity (32 bytes)
is different from the write access granularity (one byte).
To handle this, the L2 cache applies a different write allocation
policy, which we named \textit{lazy fetch-on-read}, that is a compromise
between write-validate and fetch-on-write.
When a sector read request is received to a modified sector,
it first checks if the sector write-mask is complete,
i.e. all the bytes have been written to and the line is fully readable.
If so, it reads the sector, otherwise, similar to fetch-on-write,
it generates a read request for this sector and merges it with the
modified bytes.
In Figure~\ref{fig:demystiying_l2write}, the kernel runs for a single
thread, and we inserted some dummy code (not shown in figure) to prevent
compiler from register allocating the accesses.
In Figure~\ref{fig:demystiying_l2write},
a four-byte float is written at line 3.
When it reads it back at line 5, it is a miss. 
This is because the sector is not full yet.
Note that, in a write-validate policy, this should be a hit. 
Later, at line 6, reading the same four bytes and the
next four bytes are both hits, because the whole sector is fetched from the read to C[i] at line 5.

\subsection{Streaming Throughput-oriented L1 cache \label{sec:memory-l1}}

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/streaming_cache-crop.pdf}
    \caption{Our Assumed Organization for Streaming L1 Cache in Volta \label{fig:demystiying_streaming}.}
\end{figure}

The L1 cache in Volta is what NVIDIA is calling a {\em streaming cache}~\cite{voltacache}. 
It is streaming because the documentation states that it allows unlimited cache misses to be
in flight regardless the number of cache lines per cache set~\cite{v100micro}.
In other words, L1 cache throughput is not limited by cache resources (e.g, miss-status holding
registers (MSHRs)~\cite{tuck2006scalable} and cache lines). To achieve this, we change the
miss allocation policy in the L1 to be \textit{ON\_FILL} rather than \textit{ON\_MISS} to elimante
line allocaiton fails.
Further, based on our analysis from running some micro-benchmarks, 
imilar to ~\cite{nugteren2014detailed}, we find the number of MSHRs in Volta has increased
substantially compared to previous generations.
We observe that, with just two SMs running a streaming workload, Volta can fully utilize the memory system.
Also, we notice that, independent of the number of L1 configured size, the number of MSHRs available are the same,
even if more of the on-chip SRAM storage is devoted to shared memory.
Based on that, Figure~\ref{fig:demystiying_streaming} depicts our assumed organization of streaming cache.
We believe that unified cache is a plain SRAM where sectored data blocks are shared between the L1D and the CUDA
shared memory. It can be configured adaptively by the driver as we discussed earlier.
We assume that the L1D's TAG and MSHR merging functionality are combined together in a
separate table structure (TAG-MSHR table). Since, the filling policy is now \textit{ON\_FILL},
we can have more TAG entries and outstanding requests than the assigned L1D cache lines.
When a new 32B sector request generated from the coalescer is received,
it checks the TAG array. If it hits and the status is valid, it uses a block index to access the data array.
If it is a hit to a reserved sector (i.e. the status is pending),
it sets its corresponding warp bit in the merging mask (64 bits for 64 warps).
When the pending request comes back, it allocates a cache line/sector in the data block
and sets the allocated block index in the table. Then, the merged warps access the
sector, on a cycle-by-cyle basis.

%we noticed that streaming cache in Volta allows small number of cores to fully utilize the memory system as demonstrated in section \ref{case-study}. Furhter, 



%\begin{comment}
%In fact, there are no documents nor patents that discuss more details about streaming L1 cache and how it is implemented. In this case, we totally eliminate the resource reservation failing due to MSHR and cache line allocation; and thus L1 cache can send as many requests as it needs. The drawback of this approach is that we can allow redundant requests in flight. However, we noticed that HIT\_RESERVED rarely occurs in GPGPU workloads and it represents less than 1\% of requests. Further, redundant requests will only happen while the first request is pending. Once the first request returns, all the upcoming requests to the same cache line will be hit in the cache. Our modeling for L1 streaming cache shows a high correlation with real hardware as we demonstrated in figures \ref{fig:l1-cache-contention} and \ref{fig:l1-cache-throughput}.

%Based on our analysis and running micro-benchmarks similar to\cite{nugteren2014detailed}, we find that the L1 cache has a large number of miss-status handling registers (MSHRs)\cite{tuck2006scalable} compared to previous GPU generations. While Fermi L1 cache has 64 MSHRs\cite{nugteren2014detailed}, we discovered that in Pascal, each cache line has an associated MSHR entry, and the totSHRs per GPU is equal to the total number of buffers that found in the whole memory system (interconnection, L2 and DRAM).By this way, we guarantee that we will never be bottlenecked with MSHR unavailability as previous work has shown\cite{jia2014mrpb}. 


%similar to\cite{nugteren2014detailed}, we find that the L1 cache has
%a large number of miss-status holding registers (MSHRs)\cite{tuck2006scalable}
%compared to previous GPU generations. While Fermi L1 cache has 64 MSHRs\cite{nugteren2014detailed},
%we discovered that in Pascal, each cache line has an associated MSHR entry, and the total number of MSHRs
%per GPU is equal to the total number of buffers found in the whole memory system
%(interconnection, L2 and DRAM).By
% this way, we guarantee that we will never be bottlenecked with MSHR unavailability as previous work has shown\cite{jia2014mrpb}. 

==> ispass2019-subm (2)/exploration.tex <==

\section{Design Space Exploration}
\label{sec:design-space-expl}

In this section, we analyze the impact of our new memory system modeling.
In simulation, we study detailed memory system characteristics of
GPGPU workloads on a Pascal P102 architecture with GDDR5X DRAM.
%baseline that we have validated
%against real hardware in the previous section.

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/dram-read-transactions_html_1B-3_x-PASCALTITANX_1B-TITANX-P102-copyk.pdf}
    \caption{DRAM reads for New-Model versus silicon Pascal TITAN X\label{fig:dram-reads-correl}.}
\end{figure}


%We characterize our workloads into three different
%categories,
%cache-sensitive workloads (\textit{C-type}),
%streaming memory intensive workloads (\textit{M-type})
%and regular balanced workloads (\textit{B-balanced}).

%\begin{table}
% \begin{adjustwidth}{-.5in}{-.5in}
%  \begin{center}
%     \tiny
%    \scriptsize
%   \caption{Workloads used in this study} \label{table:workloads}
%    \begin{tabular}{|l|c|c|}
%        \hline
%        workload & type & input size \\\hline
%        BLK & M-type & 320 MB \\\hline
%        CONV & M-type & 16 MB \\\hline
%        FWT & M-type & 32 MB \\\hline
%        SP & M-type & 120 MB \\\hline
%        TRA & M-type & 16 MB \\\hline
%        VecAdd & M-type & 40 MB \\\hline
%        STREAM & M-type & 20 MB \\\hline
%        Copy  & M-type & 20 MB \\\hline
%        MiniFe  & M-type & 356 MB \\\hline
%        spmv  & C-type & 10 MB \\\hline
%        AMR  & C-type & 25 MB \\\hline
%        Join  & C-type & 8 MB \\\hline
%        bc  & C-type & 15 MB \\\hline
%        color\_max & C-type & 47 MB \\\hline
%        fw  & C-type & 200 MB \\\hline
%        mis  & C-type & 200 MB \\\hline
%        pagerank & C-type & 13 MB \\\hline
%        sssp  & C-type & 60 MB \\\hline
%        sssp\_ell  & C-type & 60 MB \\\hline
%        bfs  & C-type & 40 MB \\\hline
%        MM  & B-type & 32 MB \\\hline
%        HS  & B-type & 32 MB \\\hline
%        srad\_v1 & B-type & 6 MB \\\hline
%        srad\_v2  & B-type & 16 MB \\\hline
%        cns  & B-type & 64 MB \\\hline
%        Xsbench & B-type & 20  MB \\\hline
%        lulesh & B-type & 100 MB \\\hline
%    \end{tabular}
%  \end{center}
%\end{table}

\subsection{Cache Analysis \label{sec:cache-ana}}

\begin{figure*}
    \centering
    \includegraphics[width=180mm]{figs/l2cache_perf.pdf}
    \caption{Normalized performance improvement caused by sectoring the L2 cache and improving the
    write policy.\label{fig:sector_l2cache_perf}.}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=180mm]{figs/l2_cache_reqreduced.pdf}
    \caption{L2 cache policy impact on DRAM requests normalized to the baseline non-sectored cache and na\"ive write policy\label{fig:l2_cache_reqreduced}.}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=180mm]{figs/wasted_bw.pdf}
    \caption{Memory bandwidth utilization, broken down into the reasons for inactivity.\label{fig:wasted_bw}.}
\end{figure*}

In this subsection, we analyze the impact of the sectored L2 cache
with lazy fetch-on-read compared to the existing GPPGU-Sim 3.x
cache with a na\"ive write policy that fetches cache lines on write requests to fill them.
%This is what GPGPU-Sim 3.x does.
As shown in Figure~\ref{fig:sector_l2cache_perf},
sectoring the L2 and changing the write policy improves
the performance of our applications by 8\%.
The degree of performance improvement varies greatly and some
applications show a performance degradation.
Apps that show a slowdown with the improved L2 cache benefit from the
larger spatial locality of the non-sectored cache~\cite{rhu2013locality}.
The irregular workloads, such as BFS and spmv, and write intensive
workloads show a high performance improvement
with the sectored and lazy-fetch-on-read L2 cache.
Figure~\ref{fig:l2_cache_reqreduced} shows the reduction of
dram memory requests received from the L2 cache.
The figure shows a significant reduction in dram
requests, which translates to an energy and power
reduction as well.
On average, a 36\% reduction was observed
when applying the optimized L2 cache.



%Akshay: Can we show the HW value for reference?
%Its not clear what's meant by L2 cache performance



%\subsection{Memory Characteristics Analysis}

%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/latency_sens.pdf}
%    \caption{Latency Sensitivity\label{fig:latency_sens}.}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/bw_sens.pdf}
%    \caption{Bandwidth Sensitivity\label{fig:bw_sens}.}
%\end{figure}

%First, we study the latency and bandwidth sensitivity on a wide range of workloads.
%Figure~\ref{fig:latency_sens} depicts the latency sensitivity of all our apps.
%The majority of workloads are insensitive to memory latency, except for a few.
%Akshay: Previously we said all workloads have data set 2x of L2 cache
%The workloads reduction, b+tree and nw have small input size that fits in the L2 cache and show high hit rate at L2. Thus, they are sensitive to the cold misses that occur at the beginning of the kernel and thereby sensitive to latency. Figure~\ref{fig:bw_sens} depicts the bandwidth sensitivity on a wide range of GPGPU workloads. In this experiment, while we increase the memory bandwidth, we also increase the interconnection bandwidth to ensure we have enough throughput to sustain the memory requests from dram to cores. As shown in figure, the majority of workloads are sensitive to bandwidth. Increasing the memory bandwidth by 2X and 4X leads to 2.5X and 3.1X geometric mean performance improvement respectively.
%Akshay: Looks like there are quite a few apps which see improvement at 0.5xBW
%Surprisingly, some cache sensitive workloads show a performance improvement when we decease the memory bandwidth, such as bc and pagerank. We notice that reducing the memory bandwidth for these workloads leads to increasing L2 cache hit rate. Our explanation to this behavior is that reducing the bandwidth leads to increasing the latency of memory request and thereby allows the data set to reside longer in the cache before eviction and thus alleviates the thrashing that may occur in these irregular cache-sensitive workloads ~\cite{rogers2012cache}.

%Akshay: The graphs need to be labeled
%\begin{figure*}
%    \centering
%    \includegraphics[width=180mm]{figs/RBL.pdf}
%    \caption{Row Buffer Locality\label{fig:RBL}.}
%\end{figure*}

%\begin{figure*}
%    \centering
%    \includegraphics[width=180mm]{figs/BLP.pdf}
%    \caption{Bank Level Parallelism\label{fig:BLP}.}
%\end{figure*}

%Figures~\ref{fig:RBL} and ~\ref{fig:BLP} depict the row buffer locality (RBL) and bank level parallelism (BLP)
%for our workloads. In addition, figure~\ref{fig:BLP} shows the BLP\_ready which
%measures the average number of banks that have ready requests.
%Ready request means that the row buffer of this request is opened.
%For example, BLP\_ready=2, means, on average, we always have two banks
%where each has a hit-buffer request that can be serviced right-away by
%sending a column read to the row buffer.
%Akshay: Can we put the apps together in these categories?
%As shown in the figures, GPGPU workloads come with diverse memory characteristics,
%High-RBL with High-BLP, High-RBL with Low-BLP
%and Low-RBL and High-BLP.
%Moreover, the BLP\_ready for many applications equals two.

\subsection{Memory Analysis}



\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/writebuffer-crop.pdf}
    \caption{Write Buffer Performance\label{fig:writebuffer_perf}.}
\end{figure}
\end{comment}



Figure\ref{fig:wasted_bw} answers the question,
{\em where is memory bandwidth wasted?} In other words,
why are we are not able to achieve 100\% memory bandwidth utilization?
Based on our observations, there are four limiting factors that hinder
a bank to send a request to an opened row.
First, \textit{RCD}, which is defined as minimum number of clock
cycles required between opening a row of memory and accessing columns within it.
The \textit{RCD} is severe in applications that have high BLP and low RBL.
Second, read-to-write \textit{RTW} and write-to-read \textit{WTR} are other limiting factors.
Read-to-write and Write-to-read are the bus-turnaround penalty,
when switching from serving a read request to a write request, and vice
versa\cite{stuecheli2010virtual,stuecheli2010virtual,lee2010dram}.
The bus-turn-around delays are limiting factors in workloads that
are write-intensive, e.g. streaming workloads, wherein writes represent
more than 30\% of requests received by DRAM.
Third, command-command-delay \textit{CCDL} occurs when you read from
two banks that belong to the same bank group. In workloads that have
high bank-group-level parallelism, designing an intelligent memory
address mapping with advanced memory indexing\cite{zhang2000permutation}
can hide \textit{CCDL} delay.
%In our baseline architecture,
We choose the lower bits
of the bank\_Id as bank group index, since lower bits tend to have more entropy.
Further, we xor the bank\_Id bits with the lower
bits of row\_id to increase the bank-level
and bank-group-level parallelism\cite{zhang2000permutation}.

In figure\ref{fig:wasted_bw}, we characterize the wasted bandwidth
reasons on a wide range of workloads.
Although, we are using an advanced bank-group indexing,
many workloads are still limited by \textit{CCDL}.
On the workloads matvec, MM\_optimzed, SP and Xsbench,
nearly 20\% of bandwidth is wasted due to \textit{CCDL}.
\textit{RTW} and \textit{WTR} are also observed to be 
a bandwidth bottleneck for many streaming applications,
such as bfs, TRA, VecAdd, CONV, FWT, srad\_v2 and others.
In bfs, 40\% of bandwidth is wasted due to bus-turnaround time.



Many works have tried to address the bus-turnaround penalty
\cite{stuecheli2010virtual,stuecheli2010virtual,lee2010dram}.
Using separate read/write queues is a widely-used optimization technique
that splits read and write requests into different queues.
Write requests are buffered in a write queue and drained to DRAM
in a batch when the buffer reaches a specific threshold.
To study its effect on performance, we applied read/write buffer optimizations to our baseline.
We found that many workloads are insensitive to read/write buffer
optimization though they are bottlenecked by turn-around delay as
shown in figure\ref{fig:wasted_bw}.
Our investigation for these throughput workloads shows that,
there are many read requests pending in the banks' buffers when
the write buffer starts to drain the write requests.
These pending read requests interfere with write requests and
negate the read/write optimization. This behavior is unique to
throughput-oriented GPUs and does not occur as often in CPUs
that have few pending read requests at each banks' buffer when write drain starts.

%\subsection{HBM and GDDR5X Analysis}

%HBM\cite{hbmstandard2013high} and GDDR5X\cite{gddr5xstandard2013high} are two emerging DRAM memory
%technologies that support a high level of bandwidth compared to commodity DRR and GDDR5.
%The emerging memories come with new features and enhancements, such as per-bank
%refresh command and a dual-bus interface.
%In this subsection, we try to study  the new features and analyze their impacts on GPGPU workloads.

%\subsubsection{Per-bank refresh command}
%Since DRAM is based on dynamic cells, It requires periodic
%refresh operations to prevent data loss.
%It is well-known that DRAM refreshing causes a performance degradation and energy
%overhead\cite{agrawal2016clara,chang2014improving}.
%Typically, in commodity DRAM technology, refreshing is done at the rank-level
%(i.e., all banks within the rank are refreshed simultaneously and they are unavailable
%during the refresh time). It has been shown that the all-banks refresh policy has a
%huge performance and energy overhead on multi-core CPU. The per-bank (a.k.a. single-bank)
%refresh command is a new command that was firstly introduced in LPDDR3\cite{lpddr}
%to reduce memory refresh overhead.
%Instead of refreshing all banks, It refreshes a single bank
%at a time in a restrictive, sequential round-robin order.
%However, this restrictive order can refreshes a utilized bank
%that services a pending memory and prevents overlapping refreshes
%with accesses across banks\cite{chang2014improving}.
%GDDR5X and HBM support similar refresh mode with more flexibility
%and less restrictive ordering such that refresh commands can be issued to any banks in any order. Refresh overhead will be more critical in the future as HBM and GDDR5X continue to scale. There are high demands for larger memory size, especially from emerging workloads like Deep Learning\cite{rhu2016vdnn}. 

%We study the projection of refresh overhead on future HBM modules and see the effectiveness of single-bank refresh command. Table\ref{table:refresh} shows the expected refresh timing for future HBM. These numbers are adopted from\cite{hbmstandard2013high}. We implement three different refresh policies: (1) \textit{all-bank refresh} command that refreshes all banks at a time similar to commodity DRAM, (2) \textit{Round Robin} exploits the per-bank command in a restrictive round robin manner, (3) \textit{Greedy} harnesses the flexibility of HBM's per-bank refresh by refreshing banks that do not have pending request. Figure\ref{fig:refresh} shows the performance impact when applying the different refresh techniques compared to no-refresh on memory intensive workloads (M-type). As shown in figure, all-bank refresh has a severe impact on future modules, up to 6\%, 8\%, 11\%, 20\% performance loss was observed for 4Gb, 8Gb, 16Gb and 32 Gb respectively. Thanks to per-bank refreshing, the performance loss is mitigated and only 1\%, 1.2\%, 2\% and 3\% performance loss was observed with round robin scheduling. In fact, we do not observe a performance difference between applying round robin or greedy algorithm. This is because HBM modules has high number of memory banks (16-32 banks for 1Gb and 32 Gb respectively), thus the chance that the round-robin will refresh a utilized bank is very low. Moreover, as we observed in figure\ref{fig:BLP}, most of M-type workloads have BLP\_ready equals 2, which means on average, when memory is utilized, you always have at least two ready banks, so if you mistakenly refresh one of this bank in round-robin, the other ready bank will send its own request and thereby hide the refresh impact. It is important to note that while refresh does not seem to have a performance impact on future HBM, it may still cause a huge static energy consumption for periodically refreshing the rows and destroying row buffer locality. In this work, we do not implement energy model for Pascal architecture and HBM.
%We leave modeling the Energy model and studying the refreshing energy consumption for future work. 


%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/refresh.pdf}
%    \caption{Memory Refresh Impact\label{fig:refresh}.}
%\end{figure}

%\begin{table}
% \begin{adjustwidth}{-.5in}{-.5in}
%  \begin{center}
%     \tiny
%    \scriptsize
%   \caption{DRAM Refresh Timing} \label{table:refresh}

%    \begin{tabular}{|l|c|c|c|c|}
%        \hline
%        size & 4 Gb & 8 Gb & 16 Gb & 32 Gb \\\hline
%        refresh  & 1 row & 1 row & 2 rows & 4 rows\\\hline
%        tREFI & 128 cycles & 128 cycles & 128 cycles & 128 cycles \\\hline
%        tRFC & 48 & 72 & 96 & 120 \\\hline
%    \end{tabular}
%  \end{center}
%\end{table}

%\subsubsection{HBM Dual-bus interface}

%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/HBM-dual-interface.pdf}
 %   \caption{HBM Dual Interface\label{fig:HBM-dual-interface}.}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/dual_bus_eff.pdf}
%    \caption{dual bus efficiency\label{fig:dual_bus_eff}.}
%\end{figure}


%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/dual_bus_perf.pdf}
%    \caption{dual bus Performance Impact\label{fig:dual_bus_perf}.}
%\end{figure}

%Dual-bus interface is another feature that comes with HBM. In the new interface, column and row commands have separate buses such that column and row commands can be sent simultaneously to DRAM. %Figure\ref{fig:HBM-dual-interface} depicts the structure of dual-bus interface compared to single-bus interface that is used in commodity DRAM and GDDR5X. As shown in figure, 
%In single-bus interface, typically, column-to-column delay is two cycles (i.e. the data burst are sent over two cycles). Thus, there should be one cycle delay between every read/write column requests, and thereby row commands can be sent during this CCD delay cycle. In HBM, CCD equals one cycle. This is because the data bus width has increased to 128 bits and thereby reading 32 bytes requires only one cycle. Therefore, dual bus interface is used to send row command simultaneously with column command. This new interface can improve bandwidth utilization. Figure\ref{fig:dual_bus_eff} depicts the dual-bus efficiency which is measured as the percentage of the number when row and column are issued simultaneously on the dual-bus interface. %Figure\ref{fig:dual_bus_perf} shows normalized performance improvement when applying dual-bus interface. 
%It is observed that workloads that have High-BLP tend to have higher dual-bus efficiency and more performance improvement compared to other workloads.
%SP performance is increased by 6\% with dual-bus interface.

%\subsubsection{figs/GDDR5X Pseudo-independent Memory Accesses}

%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/GDDR5X_indpen_mem_access_reduced.pdf}
%    \caption{GDDR5X independent Memory access mode\label{fig:GDDR5X_indpen_mem_access}.}
%\end{figure}

%\begin{figure}
%    \centering
%%    \includegraphics[width=85mm]{figs/dram_reqs_on_real_HW.pdf}
%    \caption{DRAM reqs on real HW to demystify GDDR5X over-fetching \label{fig:dram_reqs_on_real_HW}.}
%\end{figure}

%GDDR5X\cite{gddr5xstandard2013high} minimum access granularity (a.k.a. atom size) is 64 bytes, whereas L2 cache sector size is 32 bytes. Im this case, L2 cache will read 64 bytes for every read request and thereby reduce sector cache efficiency. However, GDDR5X comes with new access mode, Pseudo-independent Memory Accesses, in which the memory controller can still issue two different 32-bytes accesses that belong to the same row page, such that one access is sent to any column at the lower part of the row page while the other is sent to any column column within that higher part of the page.
%Figure\ref{fig:GDDR5X_indpen_mem_access} depicts the pseudo-independent memory accesses mode.
%A smart memory controller is required to find and schedule two transactions in the buffer that satisfy the previous condition and reduce GDDR5X memory over-fetching. In order to study the impact of over-fetching on modern GPUs, we have run an irregular microbenchmark on different GPU hardware that employ GDDR5 as well as on Pascal TITANX P102 that uses GDDR5X.
%Figure\ref{fig:dram_reqs_on_real_HW} shows that, on GDDR5X there are more accesses than previous GDDR5-based GPUs. Our explanation is due to GDDR5X over-fetching. In fact, we find out that GDDR5x over-fetching is typically occurred in irregular workloads whereas regular workloads tend to have the expected number of accesses. Also, we observe that most of these over-fetching accesses are write accesses. In our baseline, we do not implement GDDR5X Pseudo-independent Memory access, instead we double the number of memory channels and decrease access atom\_size to 32 bytes. We leave modeling GDDR5X over-fetching and building a smart memory controller that exploits the new feature for future work. 




==> ispass2019-subm (2)/introduction.tex <==
\section{Introduction}
%How important is accuracy in massively parallel simulation?
%As architecture researchers, we have a strong desire to explore
%design spaces unencumbered by the practical constraints and minutia 
%of modeling something exactly as it was built by company X.
%However, we must remain grounded. Like all things in engineering,
%a tradeoff exists here. On the one hand, it is not our job to model
%machines exactly as they are built, on the other if we do not model
%something that can or does exist in the real world we risk either designing
%techniques that were implemented years ago, or worse, designing techniques that will never
%be useful outside of your simulator.
%In the open-source GPU simulator space, we argue that we have
%hit a tipping point where the widely used tools have not kept
%up with the rapid change of pace in industry. What's more, half-hearted
%attempts to model a modern architecture, without doing the hard work of validating
%it are dangerous and need to be avoided.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Story::

%Architects need simulators, allow us to move fast
% however, there is collateral damage in this process
% lack of modeling can make some good ideas seem like bad ideas and vice versa
% We study the effect an under-detailed memory system has on this collateral damage in GPUs
% Demonstrate one idea that appeared to be bad in the old model (out of order memory access scheduling) (good idea looks bad)
% Demonstrate one bottleneck in the old model that has been solved
% 	by different design decisions in the real machine. (Bad idea looks good)
% To demonstrate the increased accuracy of our new model to a real machine,
% we perform a rigorous counter-by-counter comparison of both the old model and
% new model showing a large increase in memory system accuracy.
% We then apply the new model to a future GPU design point: MCM and demonstrate that it
% it is accurate enough to reproduce results obtained from a recent industry paper studying
% the issue...

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In contemporary computer architecture research, simulation is commonly used to estimate
the effectiveness of a new architectural design idea. 
High-level simulators enable architects to rapidly evaluate ideas at the expense of less accurate simulation results.
Ideas that do not show promise in simulation are discarded while those that do show promise
are refined in an iterative process~\cite{CA:AQA}.
As Figure~\ref{fig:ideas} illustrates, simulation inaccuracy can
lead to the retention of design proposals with overestimated benefits,
or the rejection of design proposals with underestimated benefits.   
%Both scenarios result in what we term  ``abstraction collateral damage''. 
In one scenario promising ideas 
are throw out prematurely leading to less optimal solutions.
In the other scenario, ineffective ideas are retained longer than necessary,
leading to wasted time and effort during the architecture design process.
%In this paper we evaluate different examples of abstraction error and how it relates to the level of detail present in the simulation model.


Our paper focuses on the simulation of massively parallel architectures,
in particular GPUs. GPUs have witnessed rapid change and a widespread increase in their
adoption with the rise of GPGPU computing and machine learning.
In academia, the design of programmable accelerators
is mostly carried out through modeling new techniques in
high level GPU simulators.
%As Figure~\ref{fig:gpu-sim-study} shows,
Over the past four years, there have been approximately 20 papers
per year focusing on GPU-design at the top architecture conferences.
80\% of those papers have used today's most
popular open-source GPU simulator, GPGPU-Sim~\cite{gpgpusimmanual}.
%is used in 
%and those that use anything else.
%Figure~\ref{fig:gpu-sim-study} breaks down
The relative popularity of GPGPU-Sim can be attributed to
several factors, but it's most appealing
aspect is perhaps the accuracy with which it models
modern GPUs (relative to other open-source solutions).
Such accuracy should provide a solid basleine for studying
important architectural ideas that are relevant to
future machines.

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/ideas-crop.pdf}
    \caption{The architecture design and simulation process represented
    as a collection of good and ineffective ideas. As the level of simulation detail increases,
    the space of effective ideas shrinks and potentially moves.\label{fig:ideas} }
\end{figure}

Recent work on validating GPGPU-Sim~\cite{jain2018quantitative}
has demonstrated that there are several areas where a lack of
detail in the performance model creates a a major source of error.
However, the bulk of the error comes from the modeling of the memory system.
Building on that observation, we perform a module-by-module
redesign of the GPU's memory system, demonstrating its improved correlation with real hardware.
Our improved performance model decreases memory system error on several
key metrics over a diverse set of benchmarks by as much as $66\times$,
resulting in a $2.5\times$ reduction in execution cycle error when modeling
and NVIDIA TITAN V GPU.
Table~\ref{ta:corr} presents the average absolute error rates of the publicly
available GPGPU-Sim 3.x versus our new model~\footnote{Simulator changes described
in this paper will be released publicly}.
The GPGPU-Sim 3.x model, or {\em old model} is a faithful representation of how papers
currently scale GPGPU-Sim to update their baseline GPU, without modifying
the code. The {\em new model} represents all the changes implemented in this paper.

\begin{table}
\small
\centering
\caption{Average absolute error and correlation rates of the publicly available
GPGPU-Sim model versus our enhanced memory system model when modeling an 
NVIDIA Volta TITAN V.}
\label{ta:corr}
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{2}{*}{Statistic} & \multicolumn{2}{l|}{Mean Abs Error} & \multicolumn{2}{l|}{Correlation} \\ \cline{2-5} 
 & \begin{tabular}{@{}c@{}}Old\\Model \end{tabular} & \begin{tabular}{@{}c@{}}New\\ Model\end{tabular} & \begin{tabular}{@{}c@{}}Old\\Model \end{tabular} &\begin{tabular}{@{}c@{}}New\\ Model\end{tabular} \\ \hline
L1 Reqs & 48\% & 0.5\% & 92\% & 100\%\\ \hline
L1 Hit Ratio & 41\% & 18\% & 89\% & 93\%\\ \hline
L2 Reads & 66\% & 1\% & 49\% & 94\%\\ \hline
L2 Writes & 56\% & 1\% & 99\% & 100\%\\ \hline
L2 Read Hits & 80\% & 15\% & 68\% & 81\%\\ \hline
%L2 Write Hit Ratio & XX\% & XX\% & XX\% & XX\%\\ \hline
DRAM Reads & 89\% & 11\% & 60\% & 95\%\\ \hline
%DRAM Writes & XX\% & XX\% & XX\% & XX\%\\ \hline
Execution Cycles & 68\% & 27\% & 71\% & 96\%\\ \hline
%Dyn. Warp Insts & XX\% & XX\% & XX\% & XX\%\\ \hline
%Occupancy & XX\% & XX\% & XX\% & XX\%\\ \hline
\end{tabular}
\end{table}

To demonstrate that our new model  more closely matches
the hardware, we perform a counter-by-counter validation of the improved memory system
versus the current 3.x memory system. During the course of this analysis
we uncover a number of interesting insights into how contemporary hardware works.
We utilized every publicly available resource to construct the new memory system
model, capturing the details of what others has either disclosed or
discovered~\cite{wong2010demystifying,nugteren2014detailed,mei2017dissecting,voltacitadel}.
However, in the process of correlating the memory system we also discovered several
new, previously undocumented features.
For example, we uncovered more detailed elements of the Volta streaming L1 cache
behaviour, implemented Volta's adaptive L1 cache configuration policy,
discovered that both the L1 and L2 caches are sectored, explored the fine details of the Volta
memory coalescer and finally discovered and implemented the L2 writepolicy for GPU caches
which attempt to conserve memory bandwidth in the presence of sub-sector reads.
%XXXX Examples include, the L1 and L2 caches are both sectored, the memory-side L2 cache design
%conserves memory bandwidth with its unique write-allocation
%policy and the L1 streaming cache allows a seemingly unbounded number of requests to be in-flight.
%We model all these aspects in GPGPU-Sim and detail our findings on their effects.
%Since memory bandwidth is a major bottleneck for many GPGPU workloads,
%we go on to answer the question ''{\em where is memory bandwidth wasted}?`` By analyzing our more detailed model.
%We create a taxonomy of wasted bandwidth, based on where the memory system
%is delayed when not servicing request (detailed in Section~\ref{sec:design-space-expl}).

%We also examine the effect increasing the level of detail in the memory system 
%has on evaluating which ideas are good ideas and which ideas are less effective.
%To explore the effects of modeling the memory system more accurately,
%our paper performs a bottom-up performance counter
%validation of GPGPU-Sim against a real Pascal Titan X GPU.
%We identify the memory system as the area of primary concern
%and 

Using this more detailed model, we perform a case-study on
the effects error in the memory system can have on
architectural design decisions.
As expected, we demonstrating that some
ideas are rendered both more and less effective
using a more detailed model.
In particular, we demonstrate that out-of-order memory access 
scheduling, which appears relatively ineffective under the old model,
yields a significant performance improvement when the level of detail
in the memory system is increased to more closely match hardware.
We then go on to demonstrate that the L1 cache throughput bottleneck
present in the current version of the simulator no longer exists in
contemporary hardware.
The introduction of streaming, banked, sectored L1s with
an allocate-on-fill policy removes a key source of contention in
GPGPU-Sim's L1 cache. Consequentially, any design aimed at mitigating
this L1 throughput bottleneck will is less effective on a contemporary
GPU, which is reflected in our enhanced simulator.




%\begin{figure}
%    \centering
%    \includegraphics[width=85mm]{figs/gpgpu-sim-study-crop.pdf}
%    \caption{ Number of GPU architecture papers published in ISCA, MICRO, HPCA
%    and ASPLOS over the last 4 years, subdivided into those using GPGPU-Sim and
%    those using something else.\label{fig:gpu-sim-study} }
%\end{figure}

%The increased sensitivity we witness in the memory bandwidth suggests
%that future GPU designs will be more sensitive to system-level architectural
%changes than the current simulation models suggest.
%To study one such system level change coming to GPUs,
%we update GPGPU-Sim to support {\em Multichip Modules} (MCM)
%(a.k.a. Chiplet-based architecture). MCM disintegrates monolithic chips into several smaller chiplets that
%are connected together using an interposer or on-package
%network~\cite{jerger2014noc}.
%Using the updated model, we are able to reproduce and investigate the results
%from a recently published industrial paper on MCM design for GPUs~\cite{arunkumar2017mcm}.

%However, the last major modeling effort made in GPGPU-Sim was more than
%5 years ago, when the simulator was updated to model the now 7 year old Fermi
%architecture~\cite{Fermi}. Since then, the standard practice to model
%modern GPUs in GPGPU-Sim is to scale the configuration of the Fermi model changing
%parameters like the number of cores, clocks, memory channels, etc.. without
%performing a rigorous validation of such a configuration against modern hardware
%and without making material changes to the simulator's baseline model in code.
%%Seven years of (partially undocumented) changes to the architecture are lost on such models
%and the academic community risks reinventing the wheel, drawing incorrect conclusions and
%missing out on the potential challenges in future architectures.


%We originally started this work seeking to answer the question {\em where is memory bandwidth wasted}?
%We created a taxonomy of wasted bandwidth, based on where the memory system
%is delayed when not servicing request (detailed in Section~\ref{sec:design-space-expl}).
%However, when we tried to verify that our model looked anything like a real GPU, we encountered the
%170\% DRAM read error present in the baseline version of GPGPU-Sim 3.x. Had we not stopped
%to validate the model (using the now available, fairly accurate performance counters available on GPUs)
%we would have developed techniques without value.
%This observation caused us to work backwards, investigating the source of error from the lower levels
%of memory back up, finishing with a DRAM read error of only 6.7\%.
%After performing the analysis on our updated model, we conclude through quantitative analysis
%that the two major sources of wasted memory bandwidth in GPUs come from read-write turn around time
%and a lack of bank-group level parallelism.

%During the course of our analysis, we discovered several design decisions that were made in GPUs
%that could be interesting areas of future research. For example, both the L1 and L2 caches
%are sectored in Pascal, greatly reducing wasted memory traffic in workloads without spatial locality.
%Second, the L1 is highly is capable of generating a very large number of requests in-flight to the point
%that it appears to have a miss status holding register for every cache-line. Furthermore, 
%the aggregate L1 miss bandwidth is enough to saturate the entire interconnect, guaranteeing that
%the L1 cache is never a bandwidth bottleneck. Third, all cudaMemcopy operations access memory through
%the L2 cache, meaning that workloads with small working sets will never miss in the L2, since
%all the data will be essentially pre-loaded by the copy kernel. Finally, the write-miss allocation
%policy at the sectored L2 appears to be unique to GPUs. In an apparent effort to reduce memory traffic
%generated by L2 write requests, writes to partial sectors in the L2 cache will not fill the sector from
%the DRAM. This means L2 sectors can live in a modified, but invalid state where no read can hit on them.
%These are just some of the more interesting aspects of GPU design discovered during
%our analysis that all helped to improve the accuracy of our model and provide
%real design opportunities for architects in the future.


This paper makes the following contributions:
\begin{itemize}
%\item It demonstrates how inaccurate the current practice of scaling the Fermi-based
%GPGPU-Sim model is when attempting to model modern GPU architectures, such as Pascal.
\item It presents the most accurate open-source
GPU performance model to date, reducing the error in Volta
execution time by a factor of $2.5\times$, by reducing
error between silicon performance counters and GPGPU-Sim by $66\times$.
\item It demonstrates the effect of modeling error on architectural
design decisions made using the simulator. We concretely
demonstrate that some problems observed using the less detailed
memory model are no longer an issue in state-of-the-art machines, which 
have designed around issues like the L1 cache bottleneck but are more 
sensitive to issues like memory access scheduling.
%\item It presents a counter-by-counter validation of the GPGPU-Sim memory system
%using a bottom-up micro-benchmarking process. We use the demystifying process
%as guidance on how to redesign GPGPU-Sim for modeling future accelerators.
\item It identifies and confirms a number of architectural design 
decisions that have be made in contemporary accelerators.
We discuss the potential reasons why these decisions
were made and suggest opportunities to exploit those
decisions in future research.
%This analysis includes a new taxonomy of wasted bandwidth in GPUs, 
%derived using our validated memory model.
\item It introduces a new open-source correlator toolset that includes a simple workflow
for compiling over the GPU applications from 8 popular GPGPU benchmark suites
for CUDA versions 4.2 through 10.0, with inputs curbed for simulation.
The toolset also includes a database of real 
hardware timing and performance counters for these workloads for five different GPU
product generations and a correlation tool that allows users of
GPGPU-Sim to easily generate counter-by-counter correlation plots for
their simulator changes or their new workloads .
%It performs a memory system design space exploration, using our newly validated model.
%We present a taxonomy of wasted bandwidth in GPUs, identifying areas for improvement.
%\item It integrates Multichip module support into GPGPU-Sim, demonstrating
%that the new model can reproduce work generated from an industrial %simulator~\cite{arunkumar2017mcm}
%and gain additional insights into how future GPUs will be built.
%This analysis also highlights the bounds on which use GPGPU-Sim accurately models workloads,
%even with the updated model.
%\item XXX It updates the GPU-Wattch Power model based on the enhanced
%performance model, using convergence analysis~\cite{conv-anal} in lieu of
%the least-square method of co-efficient scaling.
%The combination of improved performance model and scaling factor creation dramatically
%reduces the effect of scaling co-efficients on the power model solution, creating
%a more versatile power model.XXX

%\item Using our newly validated model, we perform a memory system design space
%exploration, using both GDDR5x and our newly developed 
%Akshay: Can we still say this?
%(but currently unvalidated due
%to card availability) high-bandwidth memory model. We present a taxonomy of wasted bandwidth in
%the highly correlated memory system, identifying areas for improvement.
\end{itemize}

%Akshay: This can be cut short if space is a concern.
%The organization of this paper is as follows:
%Section~\ref{sec:arch} details the pascal architecture we model.% as well.
%Section~\ref{sec:exp} presents the experimental methodology.
%Section~\ref{sec:cache-demy} illustrates how we demystified the memory system.
%Section~\ref{sec:hw-correl} presents the details of our hardware correlation using the updated model.
%Section~\ref{sec:design-space-expl} uses our model to explore the memory system design space.
%Section~\ref{sec:case-study} details a case-study using the L1 cache.
%Section~\ref{sec:related} presents the related work.
%Finally, Section~\ref{sec:conclusion} concludes the paper.

==> ispass2019-subm (2)/methodology.tex <==
\section{Experimental Setup}
\label{sec:exp}

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/Volta_archi-crop.pdf}
    \caption{Volta Architecture\label{fig:volta-arch}}.
\end{figure}

%\subsection{Pascal P102}
We modified the GPGPU-Sim 3.x~\cite{bakhoda2009analyzing} extensively to model the new Volta architecture \cite{v100,v100micro}.
Figure~\ref{fig:volta-arch} depicts the Volta V100 architecture.
The new streaming multiprocessor (SM) is composed of four warp schedulers,
compared to two warp schedulers in Fermi architecture. Each warp scheduler has a dedicated register file
(RF) and its own execution unit (EU), including: single-precision floating point unit (SP),
double-precision unit (D), special-function unit (SFU),
integer unit (INT), and tensor core unit (TENSOR) to
accelerate 4x4 matrix multiplication \cite{v100}. A warp scheduler with its dedicated RF and EUs
is named sub-core \cite{v100micro}. All the four warp schedulers share the memory unit that
contains a memory coalescer unit and a unified cache.
The coalescer unit coalesces warp requests at the granularity of eight threads whether
the request is cached or non-cached. The schedulers and memory units are connected
via a fair round-robin crossbar. 

In Volta, the L1 cache and shared memory are combined together in a 128KB unified cache.
The shared memory capacity can be set to 0, 8, 16, 32, 64 or 96 KB and the remaining cache
serves as L1 data cache (minimum L1 cache capacity = 32KB).
Unlike previous generations, the driver adaptively configures the shared memory capacity for each kernel~\cite{nvidia2010programming}
such that it avoids shared memory occupancy bottlenecks. On the other hand, if a kernel does
not utilize shared memory, the whole unified cache (128KB) will be assigned to L1 cache.
The Volta V100 comes with High Bandwidth Memory (HBM) modules~\cite{o2014highlights,hbmstandard2013high}.
Each HBM memory module contains eight channels.
Memory channels, including the memory-side L2 cache, are connected with SMs throughout an on-chip crossbar.


\begin{table*}
% \begin{adjustwidth}{-.5in}{-.5in}
  \begin{center}
%     \tiny
    \scriptsize
   \caption{Volta V100 TITANV Configuration} \label{table:volta-config}

    \begin{tabular}{|l|c|c|}
        \hline
         & Old Model & New Model \\\hline
        \#SMs & 80 & 80\\\hline
        \#SM Configuration & \begin{tabular}{@{}c@{}}Warps per SM = 64, \#Schedulers per SM = 4, \\ \#Warps per Sched = 16, RF per SM = 64 KB \end{tabular} & \textbf{+Volta model (similar to fig\ref{fig:volta-arch} )} \\\hline
        \#Exec Units & 4 SPs, 4 SFUs & \textbf{+ 4 DPs, 4 INTs} \\\hline
        Memory Unit & Fermi coalescer (32 threads coalescer) & \textbf{Volta coalescer (8 threads coalescer) + Fair memory issue}\\\hline
        Shared Memory  & Programmable-specified up to 96 KB & \textbf{Adaptive (up to 96 KB)} \\\hline
        L1 cache & \begin{tabular}{@{}c@{}}32KB, 128B line, 4 ways, write-evict, turn-on-by-default \end{tabular}& \begin{tabular}{@{}c@{}} \textbf{+32B sector, adaptive cache (up to 128 KB),} \\ \textbf{Streaming cache, banked, latency = 28 cycles} \end{tabular}
\\\hline
        L2 cache &\begin{tabular}{@{}c@{}}  4.5 MB, 24 banks, 128B line, 32 ways, Write Back, \\ Naive write allocate, LRU, latency=100 cycles \end{tabular} &   \textbf{+32B sector, Lazy\_Fetch\_on\_Read, memory copy engine model},   \\\hline
        Interconnection & 40x24 crossbar, 32B flit  & \textbf{+advanced memory partition indexing (reduce partition camping)} \\\hline
        %Freq(core:inter:L2:mem)  & 1200:1200:1200:850 MHZ & the same\\\hline
        Memory Model & GDDR5 model, BW=652 GB/sec, latency=100ns & \textbf{HBM Model, dual-bus interface, Read/Write buffers, advanced bank indexing
}\\\hline
        %DRAM Timing & QDR,nbk=16,CCD=2,RAS=34 & DDR,nbk=16,CCD=1,RAS=24\\ & RP=16,RC=48,nbkgrp=4,CCDL=4, BL=16, atom\_size=64B & RP=10,RC=34,nbkgrp=4,CCDL=2, BL=2, atom\_size=32B\\\hline
    \end{tabular}
  \end{center}
\end{table*}

The public version of GPGPU-sim models the now 9 year old Fermi architecture~\cite{Fermi}.
The standard practice in GPGPU-Sim to model modern GPUs, such as Volta, is to scale the configuration
of the Fermi model by increasing parameters like the number of cores, memory channels, clocks, number of warp schedulers etc.
without performing a rigorous validation of such a configuration against modern hardware.
In this work, we made material changes to the GPGPU-sim simulator code in order to accurately model
the Volta architecture. Table~\ref{table:volta-config} details the high-level architecture of the
Volta V100 TITANV~\cite{titanv} architecture we model and validate against. The left column of the table
contains the configuration of the GPGPU-sim 3.X old model obtained by scaling the Fermi resources similar
to standard practice. The right column lists the new changes, shown in bold, made to model Volta
architecture accurately. Note that, these new changes cannot be configured in the old model,
instead it requires significant code changes. All the data shown in the table are adopted from
either publicly available documents and patents from Nvidia \cite{v100,v100micro}, or via running
extensive in-house micro-benchmarks. Section~\ref{sec:cache-demy} discusses in more detail th
micro-benchmarks and the details they uncover.
The L1 cache's  latency, indexing, number of sets and line size is adopted from ~\cite{voltacitadel}.

We implement a throughput-oriented, banked, streaming, sectored L1 cache, a sectored L2 cache with a lazy-fetch-on-read
policy that is highly correlated with the real hardware. 
Further, we model CPU-GPU memory copy engine which we found is an important factor on L2 accesses and hit rate,
since all DRAM accesses go through the L2, including CPU-GPU memory copies~\cite{keplercache}.
In order to reduce uneven accesses across memory partitions~\cite{aji2011bounding}, we add an advanced partition
indexing that xors the L2 channel bits with randomly selected bits from the higher row
and lower bank bits~\cite{liu2018get}. In the memory system, we accurately model HBM.
This includes the dual-bus interface and the new per-bank refresh command~\cite{o2014highlights,hbmstandard2013high}.
Further, we implement the well-known memory optimization techniques, bank indexing and separate read/write buffers, to reduce bank conflicts and read-write inference~\cite{stuecheli2010virtual,stuecheli2010virtual,lee2010dram,chatterjee2014managing}.


For Validation, we use a wide range of applications to ensure our new model generalizes to
a variety of workloads. We indiscriminately include all the workloads we could get to run in simulation
from
the original GPGPU-Sim paper~\cite{bakhoda2009analyzing},
Rodinia 3.1~\cite{industry30},
the CUDA SDK~\cite{cudasdk},
Parboil~\cite{industry32},
Pannotia~\cite{che2013pannotia},
Lonestar \cite{burtscher2012quantitative},
SHOC~\cite{industry29},
and a collection of DOE proxy apps~\cite{lulesch}. The sum total of which is over 1400
unique kernel launches.
All the workloads are compiled with CUDA 10 and the compute capability of Volta architecture (=sm\_70). 
We updated the simulator to execute applications compiled with sm\_70 PTX.

==> ispass2019-subm (2)/motivation.tex <==
\section{Design decision case study \label{case-study}}

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/dram-shced-new-crop.pdf}
    \caption{FR\_FCFS performance normalized to the FCFS in both old and new model.\label{fig:dram-shced} }
\end{figure}

This section presents the effect of inaccurate memory system modeling
on architectural design decisions. An inaccurate architecture model
may lead to  unrealistic issues or incorrect conclusions that are
not relevant to state-of-the-art designs already being used in industry.
This section demonstrates how our more accurate GPU model removes the well-studied
bottleneck of L1 cache throughput and opens up new research opportunities
in more advanced memory access scheduling.
%Further, It demonstrates how a more accurate model of a contemporary GPU can uncover new problems or trends that  were not as apparent in the old model.

\textbf{DRAM scheduler}: Throughput-oriented GPGPU workloads are
often sensitive to memory bandwidth.
Thus, the DRAM memory scheduler plays an important role to efficiently utilize the memory bandwidth
and improve the performance of memory-sensitive workloads.
Figure \ref{fig:dram-shced} shows the sensitivity of GPGPU workloads for
two memory scheduling policies: the na\"ive first-come first-serve scheduling (FCFS)
and the advanced out-of-order First-row-ready first-come first-serve scheduling
(FR\_FCFS) \cite{rixner2000memory}.
The data is shown for FR\_FCFS performance normalized to the FCFS in both old and new model.
As shown in figure, the memory scheduling policy seems to be more important in the new model
than the old model. In the old model, some workloads are insensitive or show little difference between the two
scheduling policies. On average, 20\% performance increase was observed when applying FR\_FCFS in the old model. 
Yet, in the new model, the memory scheduling policy seems to be more critical. Applying FR\_FCFS in the new model improves the performance by 2X on average. This is due to updating the model to use the NVIDIA Volta memory access coalescing rules and modeling  sectored and advanced write allocation policies in the L2 cache. 
Further, with the new features and capabilities of the GDDR5X and HBM such
as dual-bus interface \cite{o2014highlights}, pseudo-independent accesses\cite{gddr5xstandard2013high}
and per-bank refresh command \cite{hbmstandard2013high},
memory scheduling will become a more critical issue to investigate.
This experiment demonstrates how accurately modeling contemporary GPU hardware reveals performance issues obscured using a less accurate simulation.





\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/dram-shced-crop.pdf}
    \caption{FCFS performance normalized to the FR\_FCFS in both old and new model.\label{fig:dram-shced}. }
\end{figure}
\end{comment}

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/l1-cache-contention-crop.pdf}
    \caption{L1 cache reservation fails per kilo cycles for some microbenchmarks.\label{fig:l1-cache-contention} }
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=85mm]{figs/l1-cache-throughput2-crop.pdf}
    \caption{BW utilization of STREAM workload for TITANV HW, Old Model and New Model when L1 cache is turned On and Off\label{fig:l1-cache-throughput}. }
\end{figure}

\textbf{L1 cache throughput}: The L1 cache throughput bottleneck for GPUs has been well studied in literature \cite{jia2014mrpb,sethia2015mascar,kim2017packet,koo2017access}. Due to massive multithreading,
GPGPU L1 caches can suffer from severe resource contention
(e.g. miss status handling registers (MSHRs) and cache line allocation~\cite{jia2014mrpb}).
However, contemporary GPUs are designed such that the L1 cache is not a throughput bottleneck.
%However, they are still.
The new GPUs employ advanced architecture techniques to improve L1 cache throughput,
such as sectored, banked and streaming L1 caches (as discussed in section \ref{sec:memory-l1}).
The new L1 cache eliminates the excessive L1 cache throughput contention.
Figure \ref{fig:l1-cache-contention} depicts the L1 cache reservation fails
per kilo cycles for the new vs old model.
The new L1 model eliminates reservation fails and the
L1 cache is no longer a throughput bottleneck.
Figure \ref{fig:l1-cache-throughput} demonstrates the bandwidth utilization when we 
run a highly streaming application (STREAM) on the new and old models vs the hardware.
The figure plots results with the L1 cache on and off as we scale down the number of active cores,
while keeping memory bandwidth the same.
As shown in figure, the hardware is able to achieve 82\%, 75\% and 68\%
of the theoretical bandwidth when we run the workload on all SM cores, 4 and 2 cores respectively.
The old model is not able to achieve the same bandwidth utilization due to the L1 cache bottleneck
and inaccurate L2 cache replacement policy (as discussed in section \ref{sec:memory-l2}).
Furthermore, the L1 cache is a clear bottleneck in the old model, as turning the cache on severely
decreases memory utilization. Turning the L1 cache on in the new model has no effect on bandwidth
utilization and very closely matches the performance of the hardware.
%On the other hand, the new model is able to achieve the same utilization as the hardware
%thanks to streaming and sectored L1 cache.





==> ispass2019-subm (2)/related.tex <==


\section{Related Work }
\label{sec:related}

There are quite a few GPU simulators and instrumentation tools that are found in literature. 
Xun et al. \cite{gong2017multi2sim} model GPU Kepler architecture \cite{Kepler} that is integrated with Multi2sim simulation infrastructure \cite{ubal2012multi2sim}. The new simulator was validated using few CUDA SDK applications. Barrio et al.\cite{del2006attila} propose ATTILA which is a trace-driven GPU simulator that models the old GT200 architecture. Raghuraman et al. \cite{balasubramanian2015miaow} propose Miaow, an open source RTL implementation of the AMD Southern Islands GPGPU ISA. Jason et al. \cite{industry28} propose gem-gpu simulator in which they integrate GPGPU-sim with the well-known CPU simulator GEM5. The GPGPU-Sim memory system was replaced with GEM5 memory infrastructure.  Beckmann~\cite{beckmann2015amd,gutierrez2018lost} proposed gem5’s GPU, which models AMD GCN architecture. Kim et al.~\cite{kim2012macsim} proposed Mac-sim a trace-driven fermi-based GPU simulator based on Ocelot~\cite{diamos2010ocelot}. Stephenson et al.\cite{stephenson2015flexible} introduce SASSI, a low-level assembly-language instrumentation tool for GPUs. Numerous works tried to demystify GPU architecture and memory system details through micro-benchmarks~\cite{wong2010demystifying,nugteren2014detailed,mei2017dissecting,voltacitadel}. 

Previous works have studied the deficiencies of GPGPU-Sim infrastructure. Nowatzki et al.\cite{nowatzki2014gem5} show that GPGPU-Sim is very inaccurate in modeling some in-core parameters and connection delays. Hongwen et al.\cite{daidemand} argue that GPGPU-Sim has a very weak L1 cache model and they suggest few enhancement to improve the L1 cache throughput. Also, Nugteren\cite{nugteren2014detailed} validate GPGPU-Sim against real Fermi hardware and find that the simulator does not accurately model the L1 cache throughput, especially the  number of miss status holding registers. There have been many works in literature that claim they model Kepler, Maxwell and Pascal architectures by scaling the Fermi resource, however none of these works correlate their new model against real hardware. A recent work \cite{jain2018quantitative} shows that there is a huge gap in GPGPU-Sim memory system modeling when correlated against Pascal hardware. 
%On the other hand, 

Our new simulator demystifies and models the latest Volta architecture and shows a high correlation with real hardware, especially in memory system, on a wide range GPGPU workloads. To the best of our knowledge, this is the first work that accurately models a GPU Volta architecture in details. There are other few works\cite{chatterjee2017architecting,o2017fine} that claim they use in-house closed-source modern Pascal simulator in their experiments, however, our new simulator is open-source.
%will be an open-source publicly-available for academic GPU research community.


%GPU memory refresh

%L2 cache policy for GPU LAMAR, sector

%MRPB, compiler study of MRPB'author, CCWS

%many paper claiming employing kepler and pascal

